Finding Top-r Influential Communities under Aggregation Functions

Community search is a problem that seeks cohesive and connected subgraphs in a graph that satisfy certain topology constraints, e.g., degree constraints. The majority of existing works focus exclusively on the topology and ignore the nodes' influence in the communities. To tackle this deficiency, influential community search is further proposed to include the node's influence. Each node has a weight, namely influence value, in the influential community search problem to represent its network influence. The influence value of a community is produced by an aggregated function, e.g., max, min, avg, and sum, over the influence values of the nodes in the same community. The objective of the influential community search problem is to locate the top-r communities with the highest influence values while satisfying the topology constraints. Existing studies on influential community search have several limitations: (i) they focus exclusively on simple aggregation functions such as min, which may fall short of certain requirements in many real-world scenarios, and (ii) they impose no limitation on the size of the community, whereas most real-world scenarios do. This motivates us to conduct a new study to fill this gap. We consider the problem of identifying the top-r influential communities with/without size constraints while using more complicated aggregation functions such as sum or avg. We give a theoretical analysis demonstrating the hardness of the problems and propose efficient and effective heuristic solutions for our topr influential community search problems. Extensive experiments on real large graphs demonstrate that our proposed solution is significantly more efficient than baseline solutions.

==> extension.tex <==
% \Song{I am afraid our submission is less than $12$ pages. Maybe we could discuss non-containment community search here or local influential community search.}

\section{extension}\label{sec:extension}

In this section, we first point out that the difference between non-overlapping community search and non-containment community search. Then, we would extend our approaches to non-overlapping influential community search.

%And our solutions is easily extended to other cohesive model.

\subsection{Non-overlapping vs. Non-containment}

It has been noted in~\cite{lqym15, bclz17}, it is possible that one $k$-influential community is the subgraph of another, based on the definition of $k$-influential community. Therefore, \cite{lqym15, bclz17} have studied top-$r$ non-contained $k$-influential community. So we first recap the definition of non-contained $k$-influential community here.

\begin{definition}\label{def:non_contained}
Let $G=(V,E,w)$ be a weighted and undirected graph, $k$ denote the degree constraint, and $f$ stand for an aggregation function. if $H$ is a $k$-influential community and does not contain a $k$-influential community $\bar{H}$, such that $f(\bar{H}) > f(H)$.
\end{definition}

\begin{figure}[!t]
	\vspace{-2mm}
	\centering
	\includegraphics[height=36mm]{non_overlap.pdf}
	%	\vspace{-2mm}
	\caption{Graph $G$}
	\label{fig:non overlap}
	\vspace{-2mm}
\end{figure}

The top-$r$ non-contained $k$-influential community search problem is investigated in~\cite{lqym15, bclz17}. It is shown in~\cite{lqym15, bclz17} that all non-containment $k$-influential community is disjoint, if the aggregation function is $\min$. However, when the aggregation function is not $\min$. The result of top-$r$ non-contained $k$-influential community search are likely to be similar. Consider the following example:

\begin{example}
Let us consider Figure~\ref{fig:non overlap}. We assume that $k=2$ and aggregation function $f$ is $\avg$. Then according to Definition~\ref{def:non_contained}, we could obtain that $\{v_{12}, v_{14}, v_{15}\}$, $\{v_{12}, v_{13}, v_{14}\}$ and $\{v_{13}, v_{14}, v_{15}\}$ are all non-contained $k$-influential community. However, there exists overlap between these $k$-influential communities.
\end{example}

To avoid the inclusion between any two communities in the result, we propose the definition of non-overlapping community search here. The definition is given below:

\begin{definition}\label{def:non_overlap}
Given a weighted and undirected graph $G=(V,E,w)$, the degree constraint $k$, and integer $r$ and an aggregation function $f$. The result of top-$r$ $k$-influential community search problem is $\{ H_1$, $H_2$, $\dots$, $H_{r} \}$. For any two communities $H_{i}$ and $H_{j}$, if the intersection of two vertex sets is empty, we called the result is non-overlapping.
\end{definition}

We use the following example to illustrate Definition~\ref{def:non_overlap}.
\begin{example}
Let us reconsider Figure~\ref{fig:non overlap} again. In this case, we also assume that $k=2$ and aggregation function $f$ is $\avg$. Then, we aim to extract top-$3$ non-overlapping $k$-influential community. Then, the results are $\{v_{13}, v_{14}, v_{15}\}$, $\{v_{8}, v_{9}, v_{11}\}$ and $\{v_{6}, v_{7}, v_{10}\}$. The influence value of each community is $14$, $28/3$ and $23/3$ respectively. There is no overlaps between any two communities in the result.
\end{example}

\subsection{Non-overlapping Community Search}

In order to compute the top-$r$ non-overlapping $k$-influential community with the highest influence value, we could slightly modify Algorithm~\ref{alg:improve_framework} and Algorithm~\ref{alg:local_search}.

As for Algorithm~\ref{alg:improve_framework}, we only running Line $1$-$2$ since we will remove the components from the graph each iteration. Thus, there is no need for us to remove vertex from each component. Considering Algorithm~\ref{alg:local_search}, once some vertex set has been pushed into output influential community list $L$. We would remove the vertex set from the graph $G$. In conclusion, computing top-$r$ non-overlapping $k$-influential community is more efficient than computing top-$r$ $k$-influential community.

%\subsection{Other $k$-core models}

%\subsection{k-Influential Community Enumeration}
%
%According to the Definition~\ref{def:enum}, Theorem~\ref{thm:sum_enum} and Theorem~\ref{thm:avg_enum}, $k$-influential community enumeration is NP-hard when the aggregated function is sum or $\avg$. We propose the following Algorithm~\ref{alg:sum_global_enum} to get the top-$r$ global $k$-influential community.
%
%\begin{algorithm}[!htbp]
%  \caption{\textsc{Sum Global Enumeration}}
%  \label{alg:sum_global_enum}
%  \KwIn{A graph $G=(V,E,w)$, degree constraint $k$, threshold constraint $\tau$}
%  \KwOut{The global $k$-influential communities which satisfy threshold constraint}
%  $H^{k}(G)=(V^{k}_{H}, E^{k}_{H}, w) \leftarrow$ compute the maximal $k$-core of $G$\;
%  $\{H^{k}_{1}, H^{k}_{2}, \dots, H^{k}_{t} \} \leftarrow$ each disjoint connected components of $H^{k}(G)$\;
%  $n \leftarrow |H^{k}(G)=(V^{k}_{H}, E^{k}_{H}, w)|$\;
%  $L \leftarrow $ keep the connected components of $H^{k}(G)$ whose influence value is greater or equal to $\tau$\;
%  $R \leftarrow \emptyset$\;
%  \While{$L \neq \emptyset$}{
%     $H \leftarrow L$ pops the top element\;
%     $R.append(H)$\;
%     $T \leftarrow \emptyset$\;
%     \ForEach{$v \in H$}{
%        $H' \leftarrow$ remove $v$ from $H$\;
%        $T.append(H')$\;
%    }
%    \For{$i \leftarrow 1$ \textbf{to} $|T|$}{
%        $\{C_{1}, C_{2}, \dots, C_{m}\} \leftarrow$ compute the connected $k$-core of $T[i]$\;
%        \For{$j \leftarrow 1$ \textbf{to} $m$}{
%            \If{$f(C_j) \geq \tau$}{
%                $L.append(C_j)$\;
%            }
%        }
%    }
%  }
%  \Return $R$\;
%\end{algorithm}
%
%Nevertheless, when the aggregated function is $\avg$, we have to slightly modify the Algorithm~\ref{alg:sum_global_enum}. In line $8$, the influence value of $H$ must be larger or equal to $\tau$ could be append to the $R$. In addition, in line $16$-$17$, any connected $k$-core of $T[i]$ should be append to $L$.

% \Song{This section is similar to top-$r$ global influential community, the main difference is that global influential community enumeration problem is NP-hard when the aggregated function is sum. Maybe we could discuss it in the appendix.}

%\subsection{Non-containment Community Search}
%
%In the literature~\cite{lqym15, bclz17}, scientists study the problem of computing the top-$r$ non-containment global $k$-influential community when the aggregated function is $\min$. Thus, we discuss the problem in this section. First, we present the definition of non-containment influential community in Definition~\ref{def:non_contain}.
%
%\begin{definition}[non-containment influential community]\label{def:non_contain}
%Given a graph $G=(V,E,w)$ and an integer $k$, a $k$-influential community $H^{k}(G)$ is a non-containment influential community, if $H^{k}(G)$ does not contain a sub-$k$-influential community $H^{k}_{s}(G)$ such that $f(H^{k}_{s}(G)) > f(H^{k}(G))$.
%\end{definition}
%
%It is easy to show that there is no need to modify the algorithms mentioned in the section~\ref{sec:sum}, when the aggregated function is sum. The reason is shown in the following lemma.
%
%\begin{lemma}
%When the aggregated function is sum, any global $k$-influential community $H^{k}(G)$ cannot contain a global $k$-influential community $H^{k}_{s}(G)$ such that $f(H^{k}_{s}(G)) > f(H^{k}(G))$.
%\end{lemma}
%
%\begin{proof}
%According to the Definition~\ref{def:non_contain} and Corollary~\ref{crl:improved_sum_global_exact}, it is not difficult for us to get that any $f(H^{k}_{s}(G)) \leq f(H^{k}(G))$, if $H^{k}_{s}(G)$ is a subgraph of $H^{k}(G)$. This completes the proof.
%\end{proof}
%
%However, when the aggregated function is $\avg$, we have to check whether the new community is contained by another community which has smaller influence value than that of new community. If there exists such a community, we have to delete it.

% \subsection{Local Influential Community Search}

% \subsection{Other Community Models}



==> miss.tex <==
Here, we present the proofs to show when the aggregation function is weight density and balanced density.

\begin{theorem}\label{thm:weight_density_topr}
When \fx is weight density, the top-$r$ $k$-influential community search problem is NP-hard.
\end{theorem}

\begin{proof}
First, we set $\beta = 1$ here to show that there does not exist any algorithm could solve the top-$r$ $k$-influential community search problem in polynomial time when the aggregation function is weight density and $\beta = 1$. Given a graph $G=(V,E,w)$, we assign each vertex $v_i \in V$ with weight $0$. Then, we build another graph $G'=(V',E',w')$ by adding a new vertex $u$ that connects all vertices in $V$. We set the weight of the new vertex $u$ as $w_c$. Suppose that there exists a polynomial-time algorithm to address the top-$r$ $k$-influential community search problem. Then, we could determine whether there exists a ($k$-$1$)-clique since the influence value of top-$1$ $k$-influential community is $w_{c} - k$ if there exists a ($k$-$1$)-clique in graph $G$. Notably, adding any new vertex (or vertices) into such a clique would only increase the denominator of the influence value. However, the decision version of maximum clique search problem is NP-complete. It is a contradiction. Thus, top-$r$ $k$-influential community search problem is NP-hard, when \fx is weight density.
\end{proof}


\begin{theorem}\label{thm:balanced_density_topr}
When \fx is balanced density, the top-$r$ $k$-influential community search problem is NP-hard.
\end{theorem}

\begin{proof}
Given a graph $G=(V,E,w)$, we assign each vertex $v_i \in V$ with weight $1$ and $|V|=n$. Then, we build another graph $G'=(V',E',w')$ by adding a new vertex $u$ that connects all vertices in $V$. We set the weight of the new vertex $u$ as $w_c$. Suppose that there exists a polynomial-time algorithm to address the top-$r$ $k$-influential community search problem. Then, we could determine whether there exists a ($\lceil \frac{n-w_{c}}{2} \rceil$-$1$)-clique since the influence value of top-$1$ $k$-influential community is $(w_c + k) / (w_{c} + 2k -n)$, where $k = \lceil \frac{n-w_{c}}{2} \rceil$, if there exists a ($\lceil \frac{n-w_{c}}{2} \rceil$-$1$)-clique in graph $G$. Notably, adding any new vertex (or vertices) into such a clique would only increase the denominator of the influence value. However, the decision version of maximum clique search problem is NP-complete. It is a contradiction. Thus, top-$r$ $k$-influential community search problem is NP-hard, when \fx is balanced density.
\end{proof}
